MDMLP-EIA: Multi-domain Dynamic MLPs with Energy Invariant Attention for Time Series Forecasting

Time series forecasting is essential across diverse domains. While MLP-based methods have gained attention for achieving Transformer-comparable performance with fewer parameters and better robustness, they face critical limitations including loss of weak seasonal signals, capacity constraints in weight-sharing MLPs, and insufficient channel fusion in channel-independent strategies. To address these challenges, we propose MDMLP-EIA (Multi-domain Dynamic MLPs with Energy Invariant Attention) with three key innovations. First, we develop an adaptive fused dual-domain seasonal MLP that categorizes seasonal signals into strong and weak components. It employs an adaptive zero-initialized channel fusion strategy to minimize noise interference while effectively integrating predictions. Second, we introduce an energy invariant attention mechanism that adaptively focuses on different feature channels within trend and seasonal predictions across time steps. This mechanism maintains constant total signal energy to align with the decomposition-prediction-reconstruction framework and enhance robustness against disturbances. Third, we propose a dynamic capacity adjustment mechanism for channel-independent MLPs. This mechanism scales neuron count with the square root of channel count, ensuring sufficient capacity as channels increase. Extensive experiments across nine benchmark datasets demonstrate that MDMLP-EIA achieves state-of-the-art performance in both prediction accuracy and computational efficiency.

==> tables/ablation_hidden_size_overall_avg.tex <==
\begin{wraptable}{R}{0.5\textwidth}
\centering
\caption{Validation of dynamic capacity adjustment mechanism. Results are MSE and MAE averaged across four prediction lengths ($T \in \{96, 192, 336, 720\}$). For each metric column, the best performance (lowest error) across hidden sizes is in \textbf{boldface}.}
\label{tab:ablation_hidden_size_overall_avg}
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{@{}l|cc|cc|cc|cc|cc@{}} 
\toprule
\multirow{2}{*}{Hidden Size} & \multicolumn{2}{c|}{ETTh1} & \multicolumn{2}{c|}{Solar} & \multicolumn{2}{c|}{Traffic} & \multicolumn{2}{c|}{Weather} & \multicolumn{2}{c}{Average} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
 & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE \\
\midrule
32   & 0.448 & 0.438 & 0.261 & 0.262 & 0.610 & 0.331 & 0.240 & 0.263 & 0.389 & 0.323 \\
64   & 0.439 & 0.430 & 0.259 & 0.258 & 0.570 & 0.314 & 0.240 & 0.263 & 0.376 & 0.316 \\
128  & 0.438 & 0.427 & 0.257 & 0.254 & 0.550 & 0.302 & \textbf{0.240} & \textbf{0.260} & 0.372 & 0.311 \\
256  & 0.439 & 0.425 & 0.249 & 0.250 & 0.500 & 0.294 & \textbf{0.240} & 0.263 & 0.356 & 0.308 \\
512  & 0.440 & 0.425 & 0.249 & 0.249 & 0.490 & 0.292 & 0.240 & 0.263 & 0.354 & 0.307 \\
1024 & 0.441 & 0.425 & 0.248 & 0.240 & 0.490 & 0.289 & 0.240 & 0.264 & 0.354 & 0.304 \\
2048 & 0.443 & 0.424 & 0.254 & 0.248 & 0.490 & \textbf{0.282} & 0.240 & 0.264 & 0.357 & 0.305 \\ \hline
DCA  & \textbf{0.440} & \textbf{0.420} & \textbf{0.239} & \textbf{0.238} & \textbf{0.480} & 0.288 & \textbf{0.240} & \textbf{0.260} & \textbf{0.350} & \textbf{0.300} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{wraptable}

==> tables/ablation_x2_avg.tex <==
\begin{table}{R}{0.5\textwidth}
\centering
\caption{Ablation study on strategies for incorporating weak seasonal signals (results averaged over prediction lengths). We compare three approaches: 1)~discarding weak signals entirely (w/o weak signal), 2)~fusing them via a MLP attention (MLP), and 3)~employing our proposed adaptive zero-initialized channel fusion (AZCF). Best results for each dataset are in \textbf{boldface}. Full per-prediction length results are available in Appendix Tab.~\ref{tab:ablation_study_x2}.}
\label{tab:ablation_x2_avg}
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{@{}lcccccc@{}} 
\toprule
\multirow{2}{*}{Dataset} & \multicolumn{2}{c}{w/o Weak signal} & \multicolumn{2}{c}{MLP} & \multicolumn{2}{c}{AZCF} \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} 
                         & MSE         & MAE         & MSE         & MAE         & MSE            & MAE            \\
\midrule
ETTh1                    & 0.442       & 0.428       & 0.440       & 0.428       & \textbf{0.437} & \textbf{0.424} \\
ETTh2                    & 0.366       & 0.389       & 0.368       & 0.391       & \textbf{0.362} & \textbf{0.387} \\
ETTm1                    & \textbf{0.377} & 0.379       & 0.382       & 0.379       & 0.378          & \textbf{0.377} \\
ETTm2                    & \textbf{0.271}       & \textbf{0.314}       & \textbf{0.271}       & \textbf{0.314}       & \textbf{0.271} & \textbf{0.314} \\
Weather                  & 0.241       & 0.263       & 0.242       & 0.265       & \textbf{0.240} & \textbf{0.262} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}

==> tables/comp.tex <==

% \begin{wraptable}{R}{0.5\textwidth} % 表格靠右，宽度为文本区域的一半
% \centering
% \caption{Average per-step runtimes (ms) by method (grid lines).} % 标题稍作修改
% \scriptsize % 启用小号字体以节省空间
% \setlength{\tabcolsep}{2pt} % 保持较小的列间距
% \begin{adjustbox}{max width=\linewidth} % 确保表格内容适应分配的宽度
% % 列定义：l (Phase列)，然后 | (竖线)，接着是9个c列(方法列)，每两个c之间用|分隔。
% % @{} 用于去除表格最左和最右的额外空白。
% \begin{tabular}{@{}l|c|c|c|c|c|c|c|c|c@{}} 
%   \hline % 使用 \hline 代替 \toprule
%   Phase & 
%   \thead{DLinear} &
%   \thead{SparseTSF} & 
%   \thead{FilterNet} &
%   \thead{FreTS} &
%   \thead{FITS} &
%   \thead{Amplifier} &
%   \thead{xPatch} &
%   \thead{MDMLP-EIA} & 
%   \thead{iTransformer} \\
%   \hline % 使用 \hline 代替 \midrule
%   Training   & 0.419 & 0.570 & 1.054 & 1.023 & 1.425 & 1.654 & 2.227 & 2.649 & 3.295 \\
%   % 注意：根据您图片示例，Training 和 Inference 两行数据之间没有水平线，所以我这里也不加。
%   % 如果需要，可以在这里也加一条 \hline
%   Inference  & 0.394 & 0.508 & 0.977 & 0.927 & 1.437 & 1.549 & 1.957 & 2.228 & 2.972 \\
%   \hline % 使用 \hline 代替 \bottomrule
% \end{tabular}
% \end{adjustbox}
% \label{tab:comp} % 建议使用新的表格标签
% \end{wraptable}

% \begin{wraptable}{R}{0.5\textwidth} % 您可以根据需要调整宽度或改为标准 table 环境
% \centering
% \caption{Average per-step runtimes by method.} % 标题中可省略(ms)，因列标题已包含
% \scriptsize % 保持小号字体
% \setlength{\tabcolsep}{4pt} % 列间距可以适当调整，3列情况下4pt或5pt可能更合适
% \begin{adjustbox}{max width=\linewidth} % 确保表格内容适应分配的宽度
% % 新的列定义：l (左对齐方法名), c (居中训练时间), c (居中推理时间)
% % 使用 | 来添加垂直线，形成网格
% \begin{tabular}{l|c|c} 
%   \hline
%   Method & Training Time (ms) & Inference Time (ms) \\
%   \hline
%   DLinear       & 0.419 & 0.394 \\
%   \hline
%   SparseTSF     & 0.570 & 0.508 \\
%   \hline
%   FilterNet     & 1.054 & 0.977 \\
%   \hline
%   FreTS         & 1.023 & 0.927 \\
%   \hline
%   FITS          & 1.425 & 1.437 \\
%   \hline
%   Amplifier     & 1.654 & 1.549 \\
%   \hline
%   xPatch        & 2.227 & 1.957 \\
%   \hline
%   MDMLP-EIA     & 2.649 & 2.228 \\ 
%   \hline
%   iTransformer  & 3.295 & 2.972 \\
%   \hline
% \end{tabular}
% \end{adjustbox}
% \label{tab:comp} % 建议为修改后的表格使用新标签
% \end{wraptable}
